Greening Multi-Tenant Data Center Demand Response

Data centers have emerged as promising resources for demand response, particularly for emergency demand response (EDR), which saves the power grid from incurring blackouts during emergency situations. However, currently, data centers typically participate in EDR by turning on backup (diesel) generators, which is both expensive and environmentally unfriendly. In this paper, we focus on "greening" demand response in multi-tenant data centers, i.e., colocation data centers, by designing a pricing mechanism through which the data center operator can efficiently extract load reductions from tenants during emergency periods to fulfill energy reduction requirement for EDR. In particular, we propose a pricing mechanism for both mandatory and voluntary EDR programs, ColoEDR, that is based on parameterized supply function bidding and provides provably near-optimal efficiency guarantees, both when tenants are price-taking and when they are price-anticipating. In addition to analytic results, we extend the literature on supply function mechanism design, and evaluate ColoEDR using trace-based simulation studies. These validate the efficiency analysis and conclude that the pricing mechanism is both beneficial to the environment and to the data center operator (by decreasing the need for backup diesel generation), while also aiding tenants (by providing payments for load reductions).

==> color.tex <==

\begin{figure*}[t]
\centering
\subfigure[Social cost]{\includegraphics[width=0.23\textwidth]{./Figs/Color/Copper/SocialCost.eps}\label{fig:default:welfareLoss}}
\subfigure[Energy reduction]{\includegraphics[width=0.23\textwidth]{./Figs/Color/temp/Energy.eps} \label{fig:default:energy}}
\subfigure[Tenants' net profits]{\includegraphics[width=0.23\textwidth]{./Figs/Color/Copper/NetUtilityTenant.eps}\label{fig:default:netUtilityTenant}}
\subfigure[Operator's total cost]{\includegraphics[width=0.23\textwidth]{./Figs/Color/Copper/NetUtilityDC.eps}\label{fig:default:netUtilityDC}}\\
\subfigure[Market clearing price]{\includegraphics[width=0.23\textwidth]{./Figs/Color/temp/Price.eps} \label{fig:default:price}}
\subfigure[Tenant 1's utilization]{\includegraphics[width=0.23\textwidth]{./Figs/Color/temp/Utilization1.eps} \label{fig:default:u1}}
\subfigure[Tenant 2's utilization]{\includegraphics[width=0.23\textwidth]{./Figs/Color/temp/Utilization2.eps} \label{fig:default:u2}}
\subfigure[Tenant 3's utilization]{\includegraphics[width=0.23\textwidth]{./Figs/Color/temp/Utilization3.eps}\label{fig:default:u3}}
\caption{Performance comparison under default settings. For each group of bars, from left to right: \ouralgT, \ouralgA, \opt, and \baseline (if applicable).}\label{fig:default}
\end{figure*}

\begin{figure*}[t]
\centering
\subfigure[Social cost]{\includegraphics[width=0.23\textwidth]{./Figs/Color/temp1/SocialCost.eps}\label{fig:default:welfareLoss}}
\subfigure[Energy reduction]{\includegraphics[width=0.23\textwidth]{./Figs/Color/temp1/Energy.eps} \label{fig:default:energy}}
\subfigure[Tenants' net profits]{\includegraphics[width=0.23\textwidth]{./Figs/Color/temp1/NetUtilityTenant.eps}\label{fig:default:netUtilityTenant}}
\subfigure[Operator's total cost]{\includegraphics[width=0.23\textwidth]{./Figs/Color/temp1/NetUtilityDC.eps}\label{fig:default:netUtilityDC}}\\
\subfigure[Market clearing price]{\includegraphics[width=0.23\textwidth]{./Figs/Color/temp1/Price.eps} \label{fig:default:price}}
\subfigure[Tenant 1's utilization]{\includegraphics[width=0.23\textwidth]{./Figs/Color/temp1/Utilization1.eps} \label{fig:default:u1}}
\subfigure[Tenant 2's utilization]{\includegraphics[width=0.23\textwidth]{./Figs/Color/temp1/Utilization2.eps} \label{fig:default:u2}}
\subfigure[Tenant 3's utilization]{\includegraphics[width=0.23\textwidth]{./Figs/Color/temp1/Utilization3.eps}\label{fig:default:u3}}
\caption{Performance comparison under default settings. For each group of bars, from left to right: \ouralgT, \ouralgA, \opt, and \baseline (if applicable).}\label{fig:default}
\end{figure*}

















==> macro.tex <==

\newcommand{\mc}{\frac{\partial c_n(s_n)}{\partial s_n}}
\newcommand{\pb}{p(\mathbf{b})}
\newcommand{\qc}{\frac{\partial Q_n(b_n; \mathbf{b}_{-n})}{b_n}}
\newcommand{\mz}{\frac{\partial c_n(z)}{\partial z}}


